Video-GPT via Next Clip Diffusion

GPT has shown its remarkable success in natural language processing. However, the language sequence is not sufficient to describe spatial-temporal details in the visual world. Alternatively, the video sequence is good at capturing such details. Motivated by this fact, we propose a concise Video-GPT in this paper by treating video as new language for visual world modeling. By analogy to next token prediction in GPT, we introduce a novel next clip diffusion paradigm for pretraining Video-GPT. Different from the previous works, this distinct paradigm allows Video-GPT to tackle both short-term generation and long-term prediction, by autoregressively denoising the noisy clip according to the clean clips in the history. Extensive experiments show our Video-GPT achieves the state-of-the-art performance on video prediction, which is the key factor towards world modeling (Physics-IQ Benchmark: Video-GPT 34.97 vs. Kling 23.64 vs. Wan 20.89). Moreover, it can be well adapted on 6 mainstream video tasks in both video generation and understanding, showing its great generalization capacity in downstream. The project page is at https://zhuangshaobin.github.io/Video-GPT.github.io/.

==> tabs/abla_nclip+cfg.tex <==
\begin{table}[t]
\centering
\begin{minipage}[tl]{0.48\linewidth}
    % \vspace{0pt}
    \raggedright
    % 
    \caption{\textbf{Ablation on the number of frames in video clip during inference.}
    }
    \vspace{-0.2cm}
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|c}
        \toprule
        \textbf{Frame in Clip} & 1 & 2 & 4 & 8 & 16 & \textbf{32} 
         \\
        
        \midrule
        % \multirow{9}{*}{\shortstack[c]{DMD2}} 
        \textbf{Phy. IQ Score} & 0.00 & 6.34 & 17.42 & 28.54 & 32.72 & \textbf{33.09} \\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.00001cm}
    
    % \vspace{-0.3cm}
    \label{tab:abla_nclip}
\end{minipage}
\hfill
\begin{minipage}[tr]{0.48\linewidth}
    % \vspace{0pt}
    \raggedleft
    % 
    \caption{\textbf{Ablation on history conditioned classifier-free guidance scale.}}
    \vspace{-0.2cm}
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|c}
        \toprule
        \textbf{CFG} & 1.0 & 1.5 & 2.0 & 2.5 & \textbf{3.0} & 3.5 
         \\
        
        \midrule
        % \multirow{9}{*}{\shortstack[c]{DMD2}} 
        \textbf{Phy. IQ Score} & 25.09 & 31.96 & 32.22 & 32.65 & \textbf{32.72} & 31.88 \\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.00001cm}
    
    % \vspace{-0.3cm}
    \label{tab:abla_cfg}
\end{minipage}
\vspace{-0.3cm}
\end{table}

==> tabs/abla_pro+data.tex <==
\begin{table}[t]
\centering
\begin{minipage}[t]{0.40\linewidth}
    \vspace{0pt}
    \raggedright
    % 
    \caption{\textbf{Ablation on the number of frames sampled from origin video used for pretraining.}}
    \vspace{-0.2cm}
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c|c}
        \toprule
        \textbf{Pretrain Frame Num.} & 16 & 48 & \textbf{80}
         \\
        \midrule
        % \multirow{9}{*}{\shortstack[c]{DMD2}} 
        \textbf{Phy. IQ Score} & 22.06 & 33.09 & \textbf{34.94} \\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.01cm}
    
    % \vspace{-0.3cm}
    \label{tab:abla_nframe}
\end{minipage}
\hfill
\begin{minipage}[t]{0.27\linewidth}
    \vspace{0pt}
    \raggedleft
    % 
    \caption{\textcolor{red}{\textbf{Ablation on whether to add noise to the clean clip.}}} %%%%这五个表融合成两个表
    \vspace{-0.2cm}
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c}
        \toprule
        \textbf{Add Noise} & No & \textbf{Yes} 
         \\
        
        \midrule
        % \multirow{9}{*}{\shortstack[c]{DMD2}} 
        \textbf{Phy. IQ Score} & 32.54 & \textbf{33.09} \\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.01cm}
    
    % \vspace{-0.3cm}
    \label{tab:abla_noise}
\end{minipage}
\hfill
\begin{minipage}[t]{0.27\linewidth}
    \vspace{0pt}
    \centering
    % 
    \caption{\textbf{Ablation on the scale of dataset used for pretraining.}}
    \vspace{-0.2cm}
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c}
        \toprule
        \textbf{Dataset Size} & 1M & \textbf{70M} 
         \\
        
        \midrule
        % \multirow{9}{*}{\shortstack[c]{DMD2}} 
        \textbf{Phy. IQ Score} & 23.16 & \textbf{33.09} \\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.01cm}
    
    % \vspace{-0.3cm}
    \label{tab:abla_data}
\end{minipage}
\vspace{-0.4cm}
\end{table}

==> tabs/class_to_video.tex <==
\begin{table*}[t]
    \renewcommand{\arraystretch}{1}
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c}
        \toprule
        \textbf{Model} & \textbf{Resolution} & \textbf{Architecture} & \textbf{VAE} & \textbf{FVD↓}\\
        \midrule
        CogVideo \cite{Hong2022CogVideoLP} & 160 $\times$ 160 & Dual-channel Transformer \cite{Hong2022CogVideoLP} & 2D & 626 \\
        Latte \cite{Ma2024LatteLD} & 256 $\times$ 256 & DiT & 2D & 478 \\
        TATS \cite{Ge2022LongVG} & 128 $\times$ 128 &  Time-Sensitive Transformer \cite{Ge2022LongVG} & - & 332 \\
        OmniTokenizer  \cite{Wang2024OmniTokenizerAJ} & 256 $\times$ 256 & Vanilla Transformer & 3D & 191 \\
        VideoFusion  \cite{Luo2023VideoFusionDD} & 128 $\times$ 128 & U-Net & - & 173 \\
        MAGVITv2-AR  \cite{Yu2024LanguageMB} & - & Vanilla Transformer & 3D & 109 \\
        ACDIT \cite{Hu2024ACDiTIA} & - & DiT & 2D & 90 \\
        Make-A-Video \cite{Singer2022MakeAVideoTG} & 256 $\times$ 256 & U-Net & 2D & 81 \\
        MAGVITv2  \cite{Yu2024LanguageMB} & - & Vanilla Transformer & 3D & 58 \\
        LARP  \cite{Wang2024LARPTV} & 128 $\times$ 128 & Vanilla Transformer & 3D & 57 \\
        FAR  \cite{Yu2024LanguageMB} & 128 $\times$ 128 & DiT & 2D & 57 \\
        
        \midrule
        Video-GPT (from scratch) & 240 $\times$ 320 &  Vanilla Transformer & 2D & \textcolor{red}{XXXXX} \\
        \textbf{Video-GPT} (finetune) & 240 $\times$ 320 &  Vanilla Transformer & 2D & \textbf{61} \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Class to video quantitative comparison on the UCF-101.} }
    \label{table:c2v}
\end{table*}

==> tabs/video_classification+retrieval.tex <==
\begin{table}[t]
\centering
\begin{minipage}[tl]{1\linewidth}
    % \vspace{0pt}
    \raggedright
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c}
        \toprule
        \textbf{Method} & Top-1 Acc. 
         \\
        
        \midrule
        MemDPC \cite{Han2020MemoryaugmentedDP} & 54.1 \\
        VideoMAEv2-H \cite{Wang2023VideoMAEVS} & 56.4 \\
        \midrule
        \textbf{Video-GPT} & \textbf{58.9} \\
        
        \bottomrule
    \end{tabular}
    }
    \vspace{0.05cm}
    \caption{\textbf{Video classification linear probe quantitative comparison on the UCF-101.}}
    
    % \vspace{-0.3cm}
    \label{tab:video_classification}
\end{minipage}
\hfill
\begin{minipage}[tr]{1\linewidth}
    % \vspace{0pt}
    \raggedleft
    % \belowrulesep=0pt\aboverulesep=0pt
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c}
        \toprule
        \textbf{Method} & R@1 
         \\
        
        \midrule
        VideoCLIP \cite{Xu2021VideoCLIPCP} & 10.4 \\
        SupportSet \cite{Patrick2020SupportsetBF} & 12.7 \\
        FiT \cite{Bain2021FrozenIT} & 18.8 \\
        \midrule
        \textbf{Video-GPT} & \textbf{22.0} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{0.05cm}
    \caption{\textbf{Video retrieval zero-shot quantitative comparison on the MSR-VTT.}}
    
    % \vspace{-0.3cm}
    \label{tab:video_retrieval}
\end{minipage}
% \vspace{-0.42cm}
\end{table}
